Multiplicity of Galactic Cepheids and RR Lyrae stars from Gaia DR2 -- II. Resolved common proper motion pairs

Context. The multiplicity of classical Cepheids (CCs) and RR Lyrae stars (RRLs) is still imperfectly known, particularly for RRLs. Aims. In order to complement the close-in short orbital period systems presented in Paper I, our aim is to detect the wide, spatially resolved companions of the targets of our reference samples of Galactic CCs and RRLs. Methods. Angularly resolved common proper motion pairs were detected using a simple progressive selection algorithm to separate the most probable candidate companions from the unrelated field stars. Results. We found 27 resolved, high probability gravitationally bound systems with CCs out of 456 examined stars, and one unbound star embedded in the circumstellar dusty nebula of the long-period Cepheid RS Pup. We found seven spatially resolved, probably bound systems with RRL primaries out of 789 investigated stars, and 22 additional candidate pairs. We report in particular new companions of three bright RRLs: OV And (companion of F4V spectral type), RR Leo (M0V), and SS Oct (K2V). In addition, we discovered resolved companions of 14 stars that were likely misclassified as RRLs. Conclusions. The detection of resolved non-variable companions around CCs and RRLs facilitates the validation of their Gaia DR2 parallaxes. The possibility to conduct a detailed analysis of the resolved coeval companions of CCs and old population RRLs will also be valuable to progress on our understanding of their evolutionary path.

==> Tables/CEP-bound-table.tex <==
\begin{sidewaystable*}
 \caption{Candidate gravitationally bound companions of Cepheids. The photometry is taken from the GDR2 for the $G_\mathrm{BP}$, $G$ and $G_\mathrm{RP}$ bands \citepads{2018A&A...616A...4E}, from 2MASS for the near infrared $JHK$ bands \citepads{2006AJ....131.1163S} and from WISE for the thermal infrared $W1$, $W2$, $W3$ and $W4$ bands \citepads{2010AJ....140.1868W,2012yCat.2311....0C}.
 $E_\mathrm{BV}$ is the $E(B-V)$ color excess. The negative GDR2 parallaxes of R\,Cru ($-1.094_{0.219}$\,mas) and $\delta$\,Cep ($-1.143_{0.468}$\,mas) have been omitted. Due to their angular proximity, the listed infrared magnitudes of CE Cas AB, V1046 Cyg and S Nor correspond to their combined flux. }
 \label{cepheids-bound-table1}
 \centering
\tiny
 \renewcommand{\arraystretch}{1}
 \setlength\tabcolsep{4.0pt}
 \begin{tabular}{lrrcrrrrrrrrrrrrrrcl}
 \hline
 \hline \noalign{\smallskip}
Cepheid / GDR2 & $\varpi_\mathrm{exp}$ & $\varpi_\mathrm{G2}$ & $\mu_{\alpha,\mathrm{G2}},\,\mu_{\delta,\mathrm{G2}}$ & Sep. & Sep. & $G_\mathrm{BP}$ & $G$ & $G_\mathrm{RP}$ & $J$ & $H$ & $K$ & $W1$ & $W2$ & $W3$ & $W4$ & $E_\mathrm{BV}$ & $M_G$ & $\log T$ & Spectral \\
 & (mas) & (mas) & (mas\,a$^{-1}$) & ($\arcsec$) & (kau) & & & & & & & & & & & & & & type \\
\hline \noalign{\smallskip}
\textbf{\object{TV CMa}} & 0.477 & $ 0.343_{ 0.034}$ & $ -0.69_{ 0.06}$,$ +0.22_{ 0.05}$ & & & 11.03 & 10.24 & 9.34 & 8.16 & 7.74 & 7.48 & 7.33 & 7.34 & 7.32 & 7.11 & 0.583$^a$ & $ -3.48$ & 3.757 & F5 \\
 3044483895574944512 & & $ 0.455_{ 0.050}$ & $ -0.50_{ 0.08}$,$ +0.05_{ 0.07}$ & 6.43 & 13.5 & 16.14 & 15.77 & 14.95 & & & & & & & & & $ +2.51$ & 3.862 & F0V \\
\hline \noalign{\smallskip}
\textbf{\object{ER Car}} & 0.959 & $ 0.825_{ 0.035}$ & $ -9.72_{ 0.06}$,$ +2.48_{ 0.05}$ & & & 7.07 & 6.60 & 5.99 & 5.26 & 4.97 & 4.81 & 4.80 & 4.57 & 4.83 & 4.78 & 0.101$^a$ & $ -4.08$ & 3.749 & F5-F8Ib \\
 5339394048386734336 & & $ 0.918_{ 0.152}$ & $-10.30_{ 0.33}$,$ +3.30_{ 0.25}$ & 35.39 & 36.9 & 18.85 & 18.43 & 17.48 & & & & & & & & & $ +8.00$ & 3.678 & M0V \\
\hline \noalign{\smallskip}
\textbf{\object{CE Cas B}} & 0.343 & $ 0.262_{ 0.030}$ & $ -3.24_{ 0.05}$,$ -2.00_{ 0.06}$ & & & 11.23 & 10.65 & 9.67 & 7.78 & 7.37 & 7.17 & 6.57 & 7.00 & 6.91 & 6.68 & 0.584$^a$ & $ -3.70$ & 3.776 & G1Iab/b \\
 2011892325047232256 & & $ 0.317_{ 0.031}$ & $ -3.32_{ 0.05}$,$ -1.71_{ 0.06}$ & 2.47 & 7.2 & 11.05 & 10.51 & 9.59 &  &  &  &  &  &  &  & & $ -3.46$ & 3.791 & F8I (Ceph.) \\
\hline \noalign{\smallskip}
\textbf{\object{DF Cas}} & 0.462 & $ 0.336_{ 0.028}$ & $ -0.55_{ 0.04}$,$ -0.25_{ 0.06}$ & & & 11.15 & 10.45 & 9.65 & 8.52 & 8.11 & 7.96 & 7.75 & 7.75 & 7.71 & 7.76 & 0.595$^a$ & $ -3.40$ & 3.788 & F6-G4:\\
 465719182408531072 & & $ 0.396_{ 0.080}$ & $ -0.85_{ 0.19}$,$ -0.77_{ 0.18}$ & 16.31 & 35.3 & 18.26 & 17.25 & 16.23 & 14.66 & 13.91 & 13.74 & & & & & & $ +3.90$ & 3.676 & K3IV \\
\hline \noalign{\smallskip}
\textbf{\object{V0659 Cen}} & 1.287 & $ 0.513_{ 0.154}$ & $ -6.00_{ 0.17}$,$ -1.76_{ 0.21}$ & & & 6.90 & 6.47 & 5.86 & 5.22 & 4.94 & 4.68 & 4.57 & 4.33 & 4.56 & 4.41 & 0.134$^e$ & $ -5.32$ & 3.762 & F6/7Ib+B6V \\
 5868451109212716928 & & $ 1.384_{ 0.318}$ & $ -6.14_{ 0.50}$,$ -2.56_{ 0.61}$ & 62.22 & 48.3 & 20.54 & 19.68 & 18.04 & & & & & & & & & $+10.12$ & 2.540 & M3V \\
\hline \noalign{\smallskip}
\textbf{\object{delta Cep}} & 3.755 & $3.71_\mathrm{ 0.12}^{\dagger}$ & $+17.64_{ 0.81}$,$ +3.97_{ 0.73}$ & & & &  & & 2.87 & 2.61 & 2.35 & 0.63 & 0.51 & 2.28 & 2.13 & 0.032$^a$ & $-$ & $-$ & F5Iab: \\
 2200153214212849024 & & $ 3.393_{ 0.049}$ & $+14.09_{ 0.09}$,$ +3.79_{ 0.09}$ & 40.74 & 10.8 & 6.29 & 6.31 & 6.31 & 6.27 & 6.36 & 6.35 & 5.98 & 6.25 & 6.34 & 5.62 & & $ -1.13$ & 4.052 & B7-B8 III-IV+F0V$^g$ \\
\hline \noalign{\smallskip}
\textbf{\object{AX Cir}} & 1.917 & $ 1.774_{ 0.345}$ & $ -4.89_{ 0.44}$,$ -5.08_{ 0.52}$ & & & 6.26 & 5.73 & 5.11 & 4.25 & 3.85 & 3.76 & 3.75 &  3.38 &  3.70 &  3.60 & 0.153$^a$ & $ -3.41$ & 3.749 & F2-G2II+B4 \\
 5874031027625742848 & & $ 1.754_{ 0.374}$ & $ -5.33_{ 0.40}$,$ -4.61_{ 0.70}$ & 81.49 & 42.5 & 20.06 & 19.81 & 18.42 & & & & & & & & & $+10.68$ & 3.586 & M3.5V \\
\hline \noalign{\smallskip}
\textbf{\object{BP Cir}} & 1.700 & $ 1.024_{ 0.040}$ & $ -5.46_{ 0.05}$,$ -3.89_{ 0.07}$ & & & 7.74 & 7.31 & 6.70 & 5.84 & 5.58 & 5.44 & 5.39 & 5.21 & 5.39 & 5.30 & 0.235$^c$ & $ -3.25$ & 3.782 & F2/3II+B6V \\
 5877472464676660480 & & $ 1.525_{ 0.188}$ & $ -5.39_{ 0.31}$,$ -3.61_{ 0.39}$ & 66.30 & 39.0 & 19.90 & 18.90 & 17.77 & & & & & & & & & $ +9.32$ & 3.253 & M2V \\
\hline \noalign{\smallskip}
\textbf{\object{R Cru}} & 1.170 &  & $ -9.47_{ 0.34}$,$ -0.33_{ 0.31}$ & & & &  & & 5.35 & 5.04 & 4.90 & 4.68 & 4.43 & 4.70 & 4.63 & 0.192$^d$ & $-$ & $-$ & F6-G2Ib-II$^j$ \\
 6054935874780531328 & & $ 1.107_{ 0.089}$ & $-11.10_{ 0.28}$,$ -0.04_{ 0.13}$ & 7.70 & 6.6 & 15.88 & 15.69 & 14.57 & & & & & & & & & $ +5.44$ & 3.730 & G8V \\
\hline \noalign{\smallskip}
\textbf{\object{X Cru}} & 0.678 & $ 0.552_{ 0.046}$ & $ -5.89_{ 0.06}$,$ -0.17_{ 0.06}$ & & & 8.69 & 8.14 & 7.41 & 6.58 & 6.14 & 5.95 & 5.88 & 5.82 & 5.86 & 5.76 & 0.286$^a$ & $ -3.86$ & 3.758 & G0/2Ib \\
 6059762524642419968 & & $ 0.638_{ 0.053}$ & $ -6.03_{ 0.08}$,$ -0.20_{ 0.07}$ & 27.23 & 40.2 & 16.48 & 16.04 & 15.36 & 14.58 & 14.14 & 14.13 & & & & & & $ +4.33$ & 3.781 & G1V \\
\hline \noalign{\smallskip}
\textbf{\object{VW Cru}} & 0.710 & $ 0.812_{ 0.045}$ & $ -3.96_{ 0.06}$,$ -1.19_{ 0.06}$ & & & 9.98 & 9.09 & 8.13 & 6.92 & 6.35 & 6.13 & 5.95 & 5.82 & 5.88 & 5.74 & 0.675$^a$ & $ -2.95$ & 3.751 & F6II\\
 6053622508133367680 & & $ 0.708_{ 0.040}$ & $ -3.94_{ 0.04}$,$ -1.13_{ 0.04}$ & 20.43 & 28.8 & 14.58 & 14.08 & 13.40 & 12.47 & 12.22 & 12.07 & & & & & & $ +1.50$ & 3.924 & A2V\\
\hline \noalign{\smallskip}
\textbf{\object{V0532 Cyg}} & 0.727 & $ 0.590_{ 0.032}$ & $ -3.40_{ 0.06}$,$ -3.65_{ 0.06}$ & & & 9.39 & 8.73 & 7.94 & 6.86 & 6.39 & 6.25 & 6.16 & 6.04 & 6.13 & 6.04 & 0.534$^a$ & $ -3.75$ & 3.784 & F8Ib\\
 1971721839529622272 & & $ 0.648_{ 0.040}$ & $ -3.39_{ 0.05}$,$ -3.56_{ 0.05}$ & 21.18 & 29.1 & 15.11 & 14.67 & 14.07 & 13.23 & 12.97 & 12.79 & & & & & & $ +2.28$ & 3.890 & F0V\\
\hline \noalign{\smallskip}
\textbf{\object{V1046 Cyg}} & 0.372 & $ 0.296_{ 0.029}$ & $ -2.98_{ 0.05}$,$ -4.28_{ 0.05}$ & & & 12.71 & 11.65 & 10.57 & 8.98 & 8.34 & 8.10 & 7.79 & 7.77 & 7.78 & 7.81 & 1.143$^e$ & $ -3.72$ & 3.808 & F6Ib\\
 2060460708575795712 & & $ 0.356_{ 0.060}$ & $ -3.34_{ 0.16}$,$ -3.88_{ 0.10}$ & 2.48 & 6.7 & 16.19 & 15.78 & 14.57 &  &  &  &  &  &  &  & & $ +0.49$ & 4.126 & B8V\\
\hline \noalign{\smallskip}
\textbf{\object{CV Mon}} & 0.601 & $ 0.511_{ 0.041}$ & $ +0.43_{ 0.07}$,$ -0.69_{ 0.07}$ & & & 10.49 & 9.62 & 8.71 & 7.37 & 6.77 & 6.52 & 6.46 & 6.31 & 6.45 & 6.37 & 0.722$^b$ & $ -3.57$ & 3.772 & G2Ib/II \\
 3127142224816361600 & & $ 0.567_{ 0.044}$ & $ +0.47_{ 0.06}$,$ -0.84_{ 0.05}$ & 11.07 & 18.4 & 13.96 & 13.57 & 12.97 & 12.14 & 11.91 & 11.73 & & & & & & $ +0.30$ & 4.137 & B8V \\
 3127142327895572352 & & $ 0.537_{0.040}$ & $+0.46_{0.05}, -0.62_{0.05}$ & 14.20 & 23.6 & 13.91 & 13.49 & 12.88 & 12.10 & 11.86 & 11.71 & 11.05 & 11.03 & 10.33 & 8.70 & & $ +0.12$ & 4.095 & B8V\\
\hline \noalign{\smallskip}
\textbf{\object{RS Nor}} & 0.487 & $ 0.450_{ 0.046}$ & $ -2.21_{ 0.07}$,$ -3.45_{ 0.06}$ & & & 10.45 & 9.59 & 8.72 & 7.23 & 6.80 & 6.60 & 6.41 & 6.47 & 6.45 & 6.41 & 0.580$^a$ & $ -3.52$ & 3.750 & F6 \\
 5932812740361508736 & & $ 0.478_{ 0.044}$ & $ -2.48_{ 0.06}$,$ -3.37_{ 0.05}$ & 17.04 & 35.0 & 14.90 & 14.55 & 13.93 & 13.06 & 12.92 & 12.74 & & & & & & $ +1.34$ & 3.969 & A1V \\
\hline \noalign{\smallskip}
\textbf{\object{SY Nor}} & 0.429 & $ 0.429_{ 0.035}$ & $ -1.37_{ 0.06}$,$ -2.10_{ 0.05}$ & & & 9.94 & 9.05 & 8.11 & 6.69 & 6.09 & 5.82 & 5.50 & 5.49 & 5.56 & 5.38 & 0.794$^a$ & $ -4.70$ & 3.779 & F9Ib+B4.5V \\
 5884729035245399424 & & $ 0.443_{ 0.053}$ & $ -2.73_{ 0.16}$,$ -2.45_{ 0.11}$ & 2.46 & 5.7 & 12.33 & 12.11 & 11.45 &  &  &  &  &  &  &  & & $ -1.96$ & 4.418 & B2V \\
 5884729035255068800 & & $ 0.438_{ 0.066}$ & $ -2.65_{ 0.14}$,$ -2.59_{ 0.11}$ & 18.03 & 42.0 & 18.05 & 17.04 & 15.98 & 14.35 & 13.92 & 13.71 & & & & & & $ +3.42$ & 3.739 & F6V \\
\hline
\end{tabular}
\tablefoot{
$^\dagger$ The expected parallax $\varpi_\mathrm{exp}$ of $\delta$\,Cep is the mean value between HST \citepads{2002AJ....124.1695B} and Hipparcos \citepads{2007MNRAS.379..723V}.
}
\tablebib{%The color excess $E(B-V)$ has been taken from
(a): \citetads{1990ApJS...72..153F};
(b): \citetads{2013A&A...550A..70G};
(c): \citetads{2015A&A...584A..80M};
(d): \citetads{2003A&A...404..423T};
(e): \citetads{1994ApJ...429..844F};
(f): \citetads{2007A&A...476...73F};
(g): \citetads{2002AJ....124.1695B};
(h): \citetads{2008MNRAS.387L...1U};
(i): \citetads{2011AJ....142...51L};
(j): VSX database \citepads{2006SASS...25...47W};
(k): \citetads{2017A&A...600A.127K}.
}
\end{sidewaystable*}

\begin{sidewaystable*}
 \caption{Continued from Table~\ref{cepheids-bound-table1}, where the references are given.}
 \label{cepheids-bound-table2}
  \centering
\tiny
 \renewcommand{\arraystretch}{1}
 \setlength\tabcolsep{4.5pt}
  \begin{tabular}{lrrcrrrrrrrrrrrrrrcl}
 \hline
 \hline \noalign{\smallskip}
Cepheid / GDR2 & $\varpi_\mathrm{exp}$ & $\varpi_\mathrm{G2}$ & $\mu_{\alpha,\mathrm{G2}},\,\mu_{\delta,\mathrm{G2}}$ & Sep. & Sep. & $G_\mathrm{BP}$ & $G$ & $G_\mathrm{RP}$ & $J$ & $H$ & $K$ & $W1$ & $W2$ & $W3$ & $W4$ & $E_\mathrm{BV}$ & $M_G$ & $\log T$ & Spectral \\
 & (mas) & (mas) & (mas\,a$^{-1}$) & ($\arcsec$) & (kau) & & & & & & & & & & & & & & type \\
\hline \noalign{\smallskip}
\textbf{\object{QZ Nor}} & 0.556 & $ 0.503_{ 0.038}$ & $ -1.84_{ 0.07}$,$ -3.79_{ 0.06}$ & & & 9.14 & 8.64 & 7.96 & 7.00 & 6.70 & 6.54 & 6.48 & 6.47 & 6.49 & 6.41 & 0.253$^f$ & $ -3.49$ & 3.766 & F6Ib/II \\
 5932565899990412672 & & $ 0.481_{ 0.098}$ & $ -1.68_{ 0.20}$,$ -3.34_{ 0.16}$ & 16.55 & 29.8 & 18.13 & 17.92 & 16.84 & & & & & & & & & $ +5.71$ & 3.750 & K1V \\
\hline \noalign{\smallskip}
\textbf{\object{AW Per}} & 1.218 & $ 1.071_{ 0.064}$ & $ +0.29_{ 0.11}$,$ -1.30_{ 0.07}$ & & & 8.57 & 7.05 & 6.60 & 5.10 & 4.79 & 4.63 & 4.55 & 4.30 & 4.51 & 4.43 & 0.489$^f$ & $ -3.90$ & 3.640 & F8I+B6: \\
 174489098011144960 & & $ 1.075_{ 0.249}$ & $ -0.81_{ 0.32}$,$ -3.14_{ 0.40}$ & 10.27 & 8.4 & 17.83 & 17.41 & 16.28 & & & & & & & & & $ +6.37$ & 3.761 & K3.5V \\
\hline \noalign{\smallskip}
\textbf{\object{RS Pup}} & 0.536 & $0.613_{0.026}$ & $-3.55_{0.01}$,$+3.08_{0.02}$ & & & 7.64 & 6.63 & 5.75  & 4.94 & 4.16 & 4.02 &  & 3.374 & 3.438 & 3.246 & 0.496$^k$ & $-5.56$ & 3.681 & F8Iab \\
5546476755539995008 & & $0.532_{0.048}$ & $-3.61_{0.07}$,$+6.22_{0.08}$ & 43.33 & 80.8 & 16.71 & 16.24 & 15.43 & 14.54 & 14.22 & 14.04 & & & & & & $+3.59$ & 3.803 & F6V$^\star$ \\
\hline \noalign{\smallskip}
\textbf{\object{U Sgr}} & 1.669 & $ 1.489_{ 0.045}$ & $ -1.68_{ 0.08}$,$ -6.13_{ 0.07}$ & & & 7.28 & 6.53 & 5.75 & 4.48 & 3.91 & 3.93 & 3.95 & 3.65 & 3.95 & 3.86 & 0.403$^a$ & $ -3.58$ & 3.742 & G1Ib/II \\
 4092905066374437760 & & $ 1.534_{ 0.074}$ & $ -1.75_{ 0.11}$,$ -5.96_{ 0.09}$ & 71.99 & 43.1 & 10.41 & 10.16 & 9.74 & 9.28 & 9.20 & 9.10 & 9.04 & 9.11 & 8.76 & 7.72 & & $ -0.06$ & 3.989 & A0IV-V \\
 4092905203841177856 & & $ 1.490_{ 0.038}$ & $ -1.45_{ 0.07}$,$ -6.18_{ 0.07}$ & 76.96 & 46.1 & 11.40 & 11.15 & 10.73 & 10.23 & 10.09 & 10.02 & 9.86 & 9.90 & 10.10 & 8.75 & & $ +0.87$ & 3.990 & A0V \\
\hline \noalign{\smallskip}
\textbf{\object{V0350 Sgr}} & 1.141 & $ 1.015_{ 0.047}$ & $ -0.28_{ 0.09}$,$ -3.11_{ 0.08}$ & & & 7.86 & 7.30 & 6.59 & 5.69 & 5.27 & 5.12 & 5.07 & 4.91 & 4.99 & 4.92 & 0.299$^f$ & $ -3.42$ & 3.763 & F8Ib/II \\
 4080121319521641344 & & $ 1.044_{ 0.048}$ & $ -1.21_{ 0.08}$,$ -3.62_{ 0.07}$ & 29.85 & 26.2 & 12.45 & 12.28 & 11.94 & 11.54 & 11.43 & 11.35 & 11.05 & 11.00 & 10.96 & 8.36 & & $ +1.50$ & 3.989 & A2V \\
 4080121521343969024 & & $ 1.139_{ 0.145}$ & $ -1.64_{ 0.32}$,$ -3.77_{ 0.30}$ & 34.92 & 30.6 & 17.67 & 17.02 & 16.20 & 15.28 & 14.61 & 14.64 & & & & & & $ +6.58$ & 3.727 & K4.5V \\
\hline \noalign{\smallskip}
\textbf{\object{V0950 Sco}} & 1.073 & $ 0.869_{ 0.052}$ & $ -0.48_{ 0.10}$,$ -1.66_{ 0.09}$ & & & 7.49 & 7.06 & 6.44 & 5.72 & 5.44 & 5.24 & 5.18 & 5.03 & 5.17 & 5.09 & 0.254$^j$ & $ -3.91$ & 3.784 & F6Ib/II \\
 5960623340819000192 & & $ 0.922_{ 0.058}$ & $ -0.45_{ 0.10}$,$ -1.88_{ 0.09}$ & 16.07 & 15.0 & 15.53 & 15.28 & 14.50 & 12.81 & 13.35 & 13.18 & & & & & & $ +4.44$ & 3.786 & G1V \\
\hline \noalign{\smallskip}
\textbf{\object{CM Sct}} & 0.518 & $ 0.405_{ 0.065}$ & $ -1.01_{ 0.10}$,$ -1.41_{ 0.09}$ & & & 11.40 & 10.51 & 9.59 & 8.22 & 7.75 & 7.49 & 7.40 & 7.43 & 7.13 & 5.92 & 0.795$^a$ & $ -3.37$ & 3.783 & F8Ib/II \\
 4253603428053877504 & & $ 0.547_{ 0.050}$ & $ -1.48_{ 0.08}$,$ -1.56_{ 0.08}$ & 25.40 & 49.0 & 15.38 & 14.73 & 13.90 & 12.83 & 12.46 & 11.56 & 11.18 & 11.39 & 9.09 & 6.77 & & $ +1.36$ & 3.863 & A1V \\
\hline \noalign{\smallskip}
\textbf{\object{EV Sct}} & 0.556 & $ 0.526_{ 0.054}$ & $ -0.22_{ 0.09}$,$ -2.70_{ 0.08}$ & & & 10.45 & 9.66 & 8.82 & 7.55 & 7.13 & 6.96 & 6.42 & 6.78 & 6.71 & 6.50 & 0.679$^a$ & $ -3.41$ & 3.786 & G0II \\
 4156513016572003840 & & $ 0.510_{ 0.043}$ & $ -0.04_{ 0.06}$,$ -2.66_{ 0.06}$ & 24.71 & 44.4 & 13.96 & 13.62 & 13.08 & 12.36 & 11.22 & 12.00 & & & & & & $ +0.21$ & 4.189 & B9V \\
\hline \noalign{\smallskip}
\textbf{\object{Polaris}} ($\alpha$ UMi) & 7.540$^{\ddagger}$ & & $+44.48_{0.11}^{\ddagger}$,$-11.85_{0.13}^{\ddagger}$ & & & &  & & 0.80 & 0.46 & 0.46 & -1.94 & -1.47 & 0.58 & 0.57 & 0.003$^f$ & $-$ & $-$ & F7Ib-II: \\
 576402619921510144 & & $ 7.321_{ 0.028}$ & $+41.95_{ 0.06}$,$-13.67_{ 0.06}$ & 17.67 & 2.3 & 8.82 & 8.64 & 8.32 & & & & & & & & & $ +2.95$ & 3.810 & F3V$^h$ \\
\hline \noalign{\smallskip}
\textbf{\object{SX Vel}} & 0.490 & $ 0.438_{ 0.041}$ & $ -4.50_{ 0.07}$,$ +4.82_{ 0.07}$ & & & 8.66 & 8.12 & 7.42 & 6.54 & 6.11 & 5.95 & 5.87 & 5.71 & 5.83 & 5.81 & 0.349$^a$ & $ -4.56$ & 3.776 & F8II \\
 5329838158460399488 & & $ 0.461_{ 0.068}$ & $ -4.83_{ 0.15}$,$ +4.50_{ 0.16}$ & 15.64 & 31.9 & 17.47 & 17.01 & 16.33 & 15.39 & 15.15 & 14.94 & & & & & & $ +4.43$ & 3.791 & G1V \\
\hline \noalign{\smallskip}
\textbf{\object{CS Vel}} & 0.292 & $ 0.194_{ 0.030}$ & $ -4.56_{ 0.06}$,$ +3.10_{ 0.06}$ & & & 12.04 & 11.19 & 10.21 & 8.79 & 8.30 & 8.07 & 7.81 & 7.81 & 7.80 & 7.37 & 0.737$^i$ & $ -4.13$ & 3.767 & G1I \\
 5308893046071732096 & & $ 0.251_{ 0.048}$ & $ -4.61_{ 0.10}$,$ +3.16_{ 0.08}$ & 10.40 & 35.6 & 16.62 & 16.20 & 15.54 & 14.66 & 14.42 & 14.26 & & & & & & $ +1.14$ & 4.070 & A0V \\
\hline \noalign{\smallskip}
\textbf{\object{DK Vel}} & 0.431 & $ 0.238_{ 0.025}$ & $ -4.07_{ 0.05}$,$ +3.62_{ 0.05}$ & & & 10.91 & 10.40 & 9.74 & 8.87 & 8.51 & 8.40 & 8.31 & 8.31 & 8.30 & 8.38 & 0.287$^i$ & $ -3.45$ & 3.774 & F8II \\
 5311599390863537408 & & $ 0.402_{ 0.089}$ & $ -3.97_{ 0.21}$,$ +3.63_{ 0.22}$ & 21.32 & 49.5 & 18.57 & 18.08 & 17.39 & & & & & & & & & $ +5.37$ & 3.771 & K0V \\
 \hline
\end{tabular}
\tablefoot{$^\ddagger$ The expected parallax $\varpi_\mathrm{exp}$ and the proper motion of Polaris are from \citetads{2007ASSL..350.....V}. $^\star$ The companion of \object{RS Pup} is an unbound field star embedded in the circumstellar nebula of the Cepheid (Sect.~\ref{rspup}).}
\end{sidewaystable*}



==> Tables/CEP-near-table.tex <==
\begin{sidewaystable*}
 \caption{Candidate \texttt{Near} companions of Cepheids, up to a maximum projected separation of 50\,kau.
Part of the listed targets also host a candidate \texttt{Bound} companion, listed in Table~\ref{cepheids-bound-table1}, where the references for the photometry are also listed.
The adopted color excesses $E(B-V)$ are taken essentially from \citetads{1990ApJS...72..153F,1994ApJ...429..844F}.}
 \label{cepheids-near-table1}
 \centering
\tiny
 \renewcommand{\arraystretch}{1}
 \setlength\tabcolsep{4.0pt}
 \begin{tabular}{lrrcrrrrrrrrrrrrrrcl}
 \hline
 \hline \noalign{\smallskip}
Cepheid / GDR2 & $\varpi_\mathrm{exp}$ & $\varpi_\mathrm{G2}$ & $\mu_{\alpha,\mathrm{G2}},\,\mu_{\delta,\mathrm{G2}}$ & Sep. & Sep. & $G_\mathrm{BP}$ & $G$ & $G_\mathrm{RP}$ & $J$ & $H$ & $K$ & $W1$ & $W2$ & $W3$ & $W4$ & $E_\mathrm{BV}$ & $M_G$ & $\log T$ &  \\
 & (mas) & (mas) & (mas\,a$^{-1}$) & ($\arcsec$) & (kau) & & & & & & & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{FF Aql}} & 2.048 & $ 1.839_{ 0.107}$ & $ -1.01_{ 0.16}$,$ -9.80_{ 0.17}$ & & & 5.73 & 5.18 & 4.58 & 4.03 & 3.74 & 3.53 & 3.51 & 2.94 & 3.42 & 3.38 & 0.224 & $ -4.07$ & 3.765 & \\
 4514145597469864192 & & $ 2.082_{ 0.449}$ & $ -3.76_{ 1.35}$,$ -4.46_{ 1.62}$ & 95.96 & 46.9 & 20.45 & 20.33 & 19.18 & & & & & & & & & $+11.37$ & 3.745 & \\
\hline \noalign{\smallskip}
\textbf{\object{V0916 Aql}} & 0.325 & $ 0.506_{ 0.050}$ & $ -1.65_{ 0.08}$,$ -5.06_{ 0.07}$ & & & 11.17 & 10.06 & 8.98 & 7.56 & 6.95 & 6.72 & 5.80 & 6.17 & 6.23 & 6.23 & 0.761 & $ -3.11$ & 3.694 & \\
 4313179507877107072 & & $ 0.347_{ 0.048}$ & $ -2.27_{ 0.13}$,$ -5.89_{ 0.12}$ & 3.45 & 10.6 & 14.43 & 13.50 & 12.30 & & & & & & & & & $ -0.51$ & 3.711 & \\
\hline \noalign{\smallskip}
\textbf{\object{eta Aql}} & 3.755 & $ 2.641_{ 0.485}$ & $ +7.67_{ 0.84}$,$ -8.84_{ 0.78}$ & & & & 7.01 & & 2.35 & 1.89 & 1.79 & 0.04 & -0.30 & 1.89 & 1.82 & 0.035 &  & & \\
 4240272815933813888 & & $ 3.361_{ 0.785}$ & $ +3.86_{ 3.00}$,$ +0.73_{ 2.47}$ & 135.78 & 36.2 & 19.92 & 20.49 & 19.40 & & & & & & & & & $+13.02$ & 3.817 & \\
\hline \noalign{\smallskip}
\textbf{\object{CK Cam}} & 1.959 & $ 1.301_{ 0.035}$ & $ +4.27_{ 0.05}$,$ -3.03_{ 0.05}$ & & & 7.76 & 7.18 & 6.45 & 5.44 & 5.12 & 4.96 & 5.01 & 4.81 & 4.95 & 4.89 & 0.501 & $ -3.53$ & 3.798 & \\
 279381953248087808 & & $ 1.670_{ 0.144}$ & $ +9.37_{ 0.27}$,$ -8.69_{ 0.25}$ & 76.53 & 39.1 & 19.89 & 18.46 & 17.22 & 15.45 & 14.71 & 14.51 & 14.20 & 14.31 & 12.76 & 9.05 & & $ +8.58$ & 3.006 & \\
\hline \noalign{\smallskip}
\textbf{\object{Y Car}} & 0.695 & $ 0.330_{ 0.036}$ & $ -9.10_{ 0.07}$,$ +2.43_{ 0.07}$ & & & 8.38 & 8.04 & 7.52 & 6.80 & 6.57 & 6.48 & 6.41 & 6.37 & 6.39 & 6.19 & 0.178 & $ -4.84$ & 3.796 & \\
 5351428787238024576 & & $ 0.718_{ 0.144}$ & $ -5.88_{ 0.34}$,$ +2.75_{ 0.31}$ & 22.47 & 32.3 & 19.08 & 18.47 & 17.49 & & & & & & & & & $ +7.34$ & 3.632 & \\
\hline \noalign{\smallskip}
\textbf{\object{UX Car}} & 0.710 & $ 0.590_{ 0.038}$ & $ -7.08_{ 0.06}$,$ +2.40_{ 0.06}$ & & & 8.65 & 8.27 & 7.71 & 7.10 & 6.87 & 6.71 & 6.48 & 6.44 & 6.49 & 6.11 & 0.123 & $ -3.20$ & 3.772 & \\
 5351721944542867072 & & $ 0.775_{ 0.086}$ & $ -8.45_{ 0.17}$,$ +3.13_{ 0.16}$ & 26.63 & 37.5 & 18.20 & 17.54 & 16.71 & 15.04 & 14.24 & 14.79 & & & & & & $ +6.70$ & 3.642 & \\
\hline \noalign{\smallskip}
\textbf{\object{UZ Car}} & 0.437 & $ 0.403_{ 0.028}$ & $ -6.23_{ 0.05}$,$ +2.92_{ 0.06}$ & & & 10.87 & 9.11 & 8.45 & 7.57 & 7.22 & 7.08 & 6.95 & 7.08 & 7.01 & 6.76 & 0.187 & $ -3.24$ & 2.788 & \\
 5254298479854443392 & & $ 0.484_{ 0.112}$ & $ -4.37_{ 0.26}$,$ +1.91_{ 0.30}$ & 20.85 & 47.7 & 18.55 & 18.29 & 17.48 & & & & & & & & & $ +6.24$ & 3.767 & \\
\hline \noalign{\smallskip}
\textbf{\object{XY Car}} & 0.366 & $ 0.359_{ 0.027}$ & $ -5.18_{ 0.05}$,$ +3.28_{ 0.05}$ & & & 9.65 & 8.97 & 8.17 & 6.96 & 6.44 & 6.17 & 6.05 & 6.01 & 6.01 & 5.92 & 0.417 & $ -4.28$ & 3.755 & \\
 5240441472232303744 & & $ 0.371_{ 0.045}$ & $ -6.39_{ 0.07}$,$ +3.49_{ 0.06}$ & 17.84 & 48.7 & 16.45 & 16.02 & 15.41 & 14.46 & 14.40 & 14.23 & & & & & & $ +2.75$ & 3.829 & \\
\hline \noalign{\smallskip}
\textbf{\object{ER Car}} & 0.959 & $ 0.825_{ 0.035}$ & $ -9.72_{ 0.06}$,$ +2.48_{ 0.05}$ & & & 7.07 & 6.60 & 5.99 & 5.26 & 4.97 & 4.81 & 4.80 & 4.57 & 4.83 & 4.78 & 0.101 & $ -4.08$ & 3.749 & \\
 5339393979667360512 & & $ 0.842_{ 0.114}$ & $ -6.15_{ 0.22}$,$ +2.08_{ 0.19}$ & 12.94 & 13.5 & 17.82 & 17.68 & 16.64 & & & & & & & & & $ +7.05$ & 3.730 & \\
\hline \noalign{\smallskip}
\textbf{\object{EY Car}} & 0.446 & $ 0.360_{ 0.025}$ & $ -6.26_{ 0.05}$,$ +3.27_{ 0.05}$ & & & 10.67 & 10.10 & 9.38 & 8.28 & 7.94 & 7.80 & 7.70 & 7.71 & 7.66 & 7.57 & 0.352 & $ -3.01$ & 3.770 & \\
 5254070090673424768 & & $ 0.395_{ 0.046}$ & $ -5.62_{ 0.08}$,$ +3.30_{ 0.07}$ & 18.39 & 41.2 & 16.58 & 16.14 & 15.48 & 14.80 & 14.32 & 14.34 & & & & & & $ +3.20$ & 3.796 & \\
\hline \noalign{\smallskip}
\textbf{\object{DD Cas}} & 0.322 & $ 0.250_{ 0.029}$ & $ -1.77_{ 0.06}$,$ -1.20_{ 0.05}$ & & & 10.07 & 9.43 & 8.63 & 7.46 & 7.02 & 6.89 & 6.84 & 6.79 & 6.81 & 6.75 & 0.501 & $ -4.83$ & 3.778 & \\
 2013029941628289920 & & $ 0.335_{ 0.061}$ & $ -2.72_{ 0.14}$,$ -1.66_{ 0.09}$ & 15.82 & 49.1 & 17.50 & 16.99 & 16.31 & 15.33 & 15.04 & 14.95 & & & & & & $ +3.30$ & 3.822 & \\
\hline \noalign{\smallskip}
\textbf{\object{VW Cen}} & 0.256 & $ 0.249_{ 0.031}$ & $ -6.03_{ 0.05}$,$ -1.17_{ 0.05}$ & & & 10.78 & 9.87 & 8.98 & 7.70 & 7.08 & 6.82 & 6.62 & 6.86 & 6.79 & 6.08 & 0.448 & $ -4.18$ & 3.691 & \\
 5864955727374022656 & & $ 0.243_{ 0.057}$ & $ -6.84_{ 0.08}$,$ -1.22_{ 0.09}$ & 10.41 & 40.7 & 17.21 & 16.79 & 16.07 & & & & & & & & & $ +2.54$ & 3.816 & \\
\hline \noalign{\smallskip}
\textbf{\object{XX Cen}} & 0.589 & $ 0.566_{ 0.042}$ & $ -4.11_{ 0.07}$,$ -1.06_{ 0.08}$ & & & 8.13 & 7.50 & 6.85 & 5.85 & 5.53 & 5.39 & 5.37 & 5.23 & 5.34 & 5.27 & 0.260 & $ -4.38$ & 3.752 & \\
 5871922301788975232 & & $ 0.646_{ 0.131}$ & $ -2.21_{ 0.30}$,$ -1.33_{ 0.37}$ & 27.82 & 47.2 & 18.70 & 18.35 & 17.45 & 16.51 & 15.82 & 15.65 & & & & & & $ +6.76$ & 3.757 & \\
\hline \noalign{\smallskip}
\textbf{\object{AY Cen}} & 0.639 & $ 0.579_{ 0.032}$ & $ -6.75_{ 0.06}$,$ +2.12_{ 0.05}$ & & & 9.14 & 8.55 & 7.83 & 6.78 & 6.45 & 6.28 & 6.22 & 6.15 & 6.23 & 6.24 & 0.310 & $ -3.41$ & 3.759 & \\
 5334506135103632768 & & $ 0.551_{ 0.107}$ & $ -5.66_{ 0.26}$,$ +1.38_{ 0.18}$ & 27.34 & 42.8 & 18.55 & 18.05 & 17.20 & & & & & & & & & $ +5.99$ & 3.753 & \\
\hline \noalign{\smallskip}
\textbf{\object{AV Cir}} & 1.802 & $ 1.045_{ 0.036}$ & $ -3.42_{ 0.04}$,$ -2.22_{ 0.06}$ & & & 7.67 & 7.14 & 6.46 & 5.58 & 5.23 & 5.11 & 5.03 & 4.81 & 5.02 & 4.95 & 0.397 & $ -3.79$ & 3.791 & \\
 5848499882282952960 & & $ 1.806_{ 0.041}$ & $-10.14_{ 0.04}$,$ -6.50_{ 0.05}$ & 89.64 & 49.7 & 14.89 & 14.43 & 13.80 & 13.02 & 12.61 & 12.51 & & & & & & $ +4.67$ & 3.811 & \\
\hline \noalign{\smallskip}
\textbf{\object{AX Cir}} & 1.917 & $ 1.774_{ 0.345}$ & $ -4.89_{ 0.44}$,$ -5.08_{ 0.52}$ & & & 6.26 & 5.73 & 5.11 & 4.25 & 3.85 & 3.76 & 3.75 & 3.38 & 3.70 & 3.60 & 0.153 & $ -3.41$ & 3.749 & \\
 5874030958906259072 & & $ 1.857_{ 0.406}$ & $ -7.45_{ 0.49}$,$ -4.66_{ 0.82}$ & 44.15 & 23.0 & 18.95 & 18.44 & 17.22 & & & & & & & & & $ +9.43$ & 3.532 & \\
\hline \noalign{\smallskip}
\textbf{\object{BP Cir}} & 1.700 & $ 1.024_{ 0.040}$ & $ -5.46_{ 0.05}$,$ -3.89_{ 0.07}$ & & & 7.74 & 7.31 & 6.70 & 5.84 & 5.58 & 5.44 & 5.39 & 5.21 & 5.39 & 5.30 & 0.235 & $ -3.25$ & 3.782 & \\
 5877460610633466496 & & $ 1.552_{ 0.260}$ & $ -3.61_{ 0.45}$,$ -3.54_{ 0.56}$ & 82.78 & 48.7 & 19.93 & 19.39 & 17.95 & & & & & & & & & $ +9.83$ & 3.400 & \\
 5877460782359164928 & & $ 1.837_{ 0.364}$ & $ -5.35_{ 0.63}$,$ -1.70_{ 0.81}$ & 56.99 & 33.5 & 20.20 & 19.70 & 18.36 & & & & & & & & & $+10.50$ & 3.521 & \\
 5877472430316940672 & & $ 1.506_{ 0.172}$ & $ -3.02_{ 0.29}$,$ -2.59_{ 0.35}$ & 49.45 & 29.1 & 19.34 & 18.62 & 17.54 & 15.54 & 13.87 & 13.76 & 12.24 & 12.44 & 11.93 & 8.56 & & $ +8.98$ & 3.555 & \\
\hline \noalign{\smallskip}
\textbf{\object{T Cru}} & 1.306 & $ 1.169_{ 0.028}$ & $-10.96_{ 0.05}$,$ -0.54_{ 0.05}$ & & & 6.97 & 6.41 & 5.76 & 4.93 & 4.62 & 4.44 & 4.26 & 4.09 & 4.35 & 4.24 & 0.193 & $ -3.74$ & 3.749 & \\
 6054829771915831808 & & $ 1.254_{ 0.050}$ & $-14.26_{ 0.09}$,$ -1.33_{ 0.07}$ & 46.43 & 35.6 & 17.10 & 16.46 & 15.67 & 14.70 & 14.09 & 14.16 & & & & & & $ +6.50$ & 3.698 & \\
\hline \noalign{\smallskip}
\textbf{\object{X Cru}} & 0.678 & $ 0.552_{ 0.046}$ & $ -5.89_{ 0.06}$,$ -0.17_{ 0.06}$ & & & 8.69 & 8.14 & 7.41 & 6.58 & 6.14 & 5.95 & 5.88 & 5.82 & 5.86 & 5.76 & 0.286 & $ -3.86$ & 3.758 & \\
 6059763997807862656 & & $ 0.677_{ 0.128}$ & $ -6.06_{ 0.21}$,$ +0.42_{ 0.23}$ & 21.68 & 32.0 & 18.75 & 18.22 & 17.46 & & & & & & & & & $ +6.66$ & 3.757 & \\
\hline \noalign{\smallskip}
\textbf{\object{SU Cyg}} & 1.234 & $ 1.198_{ 0.052}$ & $ -1.79_{ 0.10}$,$ -3.28_{ 0.08}$ & & & 7.22 & 6.85 & 6.28 & 5.79 & 5.49 & 5.42 & 5.26 & 5.10 & 5.22 & 5.16 & 0.096 & $ -3.01$ & 3.767 & \\
 2031776236946397696 & & $ 1.212_{ 0.239}$ & $ -0.93_{ 0.58}$,$ -3.76_{ 0.59}$ & 42.43 & 34.4 & 19.64 & 19.23 & 18.16 & & & & & & & & & $ +9.42$ & 3.630 & \\
\hline
\end{tabular}
\end{sidewaystable*}




\begin{sidewaystable*}
 \caption{Continued from Table~\ref{cepheids-near-table1}. The negative parallax of Y Sgr ($\varpi_\mathrm{G2} = -0.441 \pm 0.280$\,mas) has been omitted.}
 \label{cepheids-near-table2}
  \centering
\tiny
 \renewcommand{\arraystretch}{1}
 \setlength\tabcolsep{4.5pt}
  \begin{tabular}{lrrcrrrrrrrrrrrrrrcl}
 \hline
 \hline \noalign{\smallskip}
Cepheid / GDR2 & $\varpi_\mathrm{exp}$ & $\varpi_\mathrm{G2}$ & $\mu_{\alpha,\mathrm{G2}},\,\mu_{\delta,\mathrm{G2}}$ & Sep. & Sep. & $G_\mathrm{BP}$ & $G$ & $G_\mathrm{RP}$ & $J$ & $H$ & $K$ & $W1$ & $W2$ & $W3$ & $W4$ & $E_\mathrm{BV}$ & $M_G$ & $\log T$ & \\
 & (mas) & (mas) & (mas\,a$^{-1}$) & ($\arcsec$) & (kau) & & & & & & & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{SZ Cyg}} & 0.419 & $ 0.391_{ 0.026}$ & $ -2.20_{ 0.05}$,$ -5.56_{ 0.06}$ & & & 9.89 & 9.03 & 8.03 & 6.39 & 5.89 & 5.71 & 5.49 & 5.45 & 5.50 & 5.60 & 0.631 & $ -4.48$ & 3.737 & \\
 2071433765909165952 & & $ 0.398_{ 0.065}$ & $ -1.98_{ 0.14}$,$ -4.54_{ 0.17}$ & 19.60 & 46.8 & 18.50 & 17.16 & 15.96 & 13.74 & 12.86 & 12.59 & & & & & & $ +3.86$ & 3.342 & \\
\hline \noalign{\smallskip}
\textbf{\object{V1334 Cyg}} & 1.502 & $ 1.180_{ 0.066}$ & $ +3.77_{ 0.10}$,$ +0.18_{ 0.12}$ & & & 6.02 & 5.75 & 5.32 & 5.17 & 4.66 & 4.46 & 4.38 & 4.06 & 4.45 & 4.38 & 0.074 & $ -4.09$ & 3.796 & \\
 1964855939153629312 & & $ 1.409_{ 0.318}$ & $ -0.37_{ 0.66}$,$ -3.27_{ 0.68}$ & 65.67 & 43.7 & 20.51 & 19.66 & 18.53 & 16.36 & 15.41 & 15.28 & & & & & & $+10.25$ & 3.184 & \\
\hline \noalign{\smallskip}
\textbf{\object{RR Lac}} & 0.515 & $ 0.352_{ 0.033}$ & $ -3.65_{ 0.06}$,$ -3.21_{ 0.06}$ & & & 9.26 & 8.73 & 7.98 & 7.14 & 6.71 & 6.58 & 6.36 & 6.31 & 6.37 & 6.33 & 0.353 & $ -4.43$ & 3.772 & \\
 2006989121667183872 & & $ 0.490_{ 0.041}$ & $ -4.78_{ 0.05}$,$ -4.53_{ 0.05}$ & 18.46 & 35.8 & 15.39 & 15.03 & 14.47 & 13.73 & 13.44 & 13.45 & & & & & & $ +2.53$ & 3.837 & \\
\hline \noalign{\smallskip}
\textbf{\object{CV Mon}} & 0.601 & $ 0.511_{ 0.041}$ & $ +0.43_{ 0.07}$,$ -0.69_{ 0.07}$ & & & 10.49 & 9.62 & 8.71 & 7.37 & 6.77 & 6.52 & 6.46 & 6.31 & 6.45 & 6.37 & 0.722 & $ -3.57$ & 3.772 & \\
 3127142220517515392 & & $ 0.594_{ 0.062}$ & $ +0.12_{ 0.12}$,$ -0.77_{ 0.12}$ & 17.70 & 29.4 & 17.19 & 16.48 & 15.65 & & & & & & & & & $ +3.52$ & 3.814 & \\
 3127142327895572352 & & $ 0.537_{ 0.040}$ & $ +0.46_{ 0.05}$,$ -0.62_{ 0.05}$ & 14.20 & 23.6 & 13.91 & 13.49 & 12.88 & 12.10 & 11.86 & 11.71 & 11.05 & 11.03 & 10.33 & 8.70 & & $ +0.12$ & 4.095 & \\
\hline \noalign{\smallskip}
\textbf{\object{S Nor}} & 1.126 & $ 1.091_{ 0.042}$ & $ -1.51_{ 0.07}$,$ -2.32_{ 0.06}$ & & & 6.82 & 6.18 & 5.55 & 4.87 & 4.50 & 4.22 & 4.08 & 3.82 & 4.01 & 3.95 & 0.189 & $ -4.10$ & 3.737 & \\
 5835124121463456896 & & $ 0.977_{ 0.052}$ & $ -1.45_{ 0.09}$,$ -2.50_{ 0.08}$ & 46.32 & 41.1 & 16.69 & 16.04 & 15.24 & 14.19 & 13.59 & 13.36 & 12.54 & 12.59 & 12.87 & 9.21 & & $ +5.54$ & 3.691 & \\
 5835124121533801088 & & $ 1.171_{ 0.097}$ & $ -2.02_{ 0.32}$,$ -1.85_{ 0.16}$ & 43.66 & 38.8 & & 17.09 & & 13.03 & 12.42 & 12.26 & 11.53 & 11.58 & 12.25 & 9.11 & &  & & \\
\hline \noalign{\smallskip}
\textbf{\object{U Nor}} & 0.699 & $ 0.641_{ 0.050}$ & $ -2.01_{ 0.10}$,$ -2.79_{ 0.09}$ & & & 9.49 & 8.43 & 7.43 & 5.77 & 5.18 & 4.91 & 4.64 & 4.44 & 4.80 & 4.67 & 0.892 & $ -4.62$ & 3.762 & \\
 5884368494207976960 & & $ 0.751_{ 0.170}$ & $ -4.36_{ 0.54}$,$ -2.47_{ 0.41}$ & 16.47 & 23.6 & 20.10 & 18.60 & 17.17 & 13.53 & 13.93 & 13.41 & & & & & & $ +6.21$ & 3.266 & \\
\hline \noalign{\smallskip}
\textbf{\object{RS Nor}} & 0.487 & $ 0.450_{ 0.046}$ & $ -2.21_{ 0.07}$,$ -3.45_{ 0.06}$ & & & 10.45 & 9.59 & 8.72 & 7.23 & 6.80 & 6.60 & 6.41 & 6.47 & 6.45 & 6.41 & 0.580 & $ -3.52$ & 3.750 & \\
 5932812431123859712 & & $ 0.480_{ 0.059}$ & $ -1.03_{ 0.09}$,$ -1.92_{ 0.07}$ & 7.55 & 15.5 & 16.31 & 15.63 & 14.67 & 11.52 & 12.82 & 11.09 & & & & & & $ +2.63$ & 3.765 & \\
\hline \noalign{\smallskip}
\textbf{\object{QZ Nor}} & 0.556 & $ 0.503_{ 0.038}$ & $ -1.84_{ 0.07}$,$ -3.79_{ 0.06}$ & & & 9.14 & 8.64 & 7.96 & 7.00 & 6.70 & 6.54 & 6.48 & 6.47 & 6.49 & 6.41 & 0.253 & $ -3.49$ & 3.766 & \\
 5932565968801321344 & & $ 0.509_{ 0.070}$ & $ -1.23_{ 0.14}$,$ -2.49_{ 0.11}$ & 27.43 & 49.3 & 17.78 & 17.23 & 16.47 & 15.80 & 16.08 & 15.94 & & & & & & $ +5.13$ & 3.745 & \\
 5932565900081828480 & & $ 0.554_{ 0.045}$ & $ -2.35_{ 0.06}$,$ -4.72_{ 0.06}$ & 16.54 & 29.7 & 13.73 & 13.36 & 12.80 & 12.07 & 11.81 & 11.79 & & & & & & $ +1.40$ & 3.801 & \\
\hline \noalign{\smallskip}
\textbf{\object{Y Oph}} & 1.850 & $ 1.390_{ 0.083}$ & $ -3.21_{ 0.14}$,$ -4.73_{ 0.11}$ & & & 7.08 & 5.60 & 4.73 & 3.67 & 3.08 & 2.82 & 1.36 & 1.17 & 2.58 & 2.47 & 0.655 & $ -5.09$ & 3.536 & \\
 4175017591096420352 & & $ 1.914_{ 0.424}$ & $ +0.30_{ 1.09}$,$ -1.00_{ 1.17}$ & 81.31 & 44.0 & 20.76 & 19.80 & 18.61 & & & & & & & & & $ +9.75$ & 3.657 & \\
\hline \noalign{\smallskip}
\textbf{\object{AQ Pup}} & 0.312 & $ 0.319_{ 0.034}$ & $ -2.57_{ 0.06}$,$ +2.57_{ 0.06}$ & & & 9.31 & 8.37 & 7.44 & 5.88 & 5.33 & 5.09 & 4.62 & 4.65 & 4.99 & 4.88 & 0.512 & $ -5.29$ & 3.694 & \\
 5597379745861712512 & & $ 0.339_{ 0.060}$ & $ -2.77_{ 0.09}$,$ +2.27_{ 0.10}$ & 9.88 & 31.7 & 16.84 & 16.45 & 15.79 & & & & & & & & & $ +2.72$ & 3.874 & \\
\hline \noalign{\smallskip}
\textbf{\object{U Sgr}} & 1.669 & $ 1.489_{ 0.045}$ & $ -1.68_{ 0.08}$,$ -6.13_{ 0.07}$ & & & 7.28 & 6.53 & 5.75 & 4.48 & 3.91 & 3.93 & 3.95 & 3.65 & 3.95 & 3.86 & 0.403 & $ -3.58$ & 3.742 & \\
 4092904791496145664 & & $ 1.562_{ 0.101}$ & $ -0.88_{ 0.24}$,$ -5.99_{ 0.22}$ & 66.82 & 40.0 & 18.53 & 17.64 & 16.55 & & & & & & & & & $ +7.71$ & 3.576 & \\
 4092904993291428864 & & $ 1.512_{ 0.286}$ & $ -4.86_{ 0.68}$,$ -6.52_{ 0.62}$ & 35.35 & 21.2 & 19.05 & 18.70 & 17.13 & 15.58 & 13.47 & 13.36 & & & & & & $ +8.70$ & 3.609 & \\
\hline \noalign{\smallskip}
\textbf{\object{Y Sgr}} & 2.146 & $-$ & $ -3.19_{ 0.37}$,$ -8.13_{ 0.28}$ & & & 7.60 & 8.23 & 6.01 & 3.92 & 3.56 & 3.50 & 3.61 & 3.34 & 3.62 & 3.61 & 0.205 & $-$ & 3.647 & \\
 4096107737550993664 & & $ 1.891_{ 0.370}$ & $ +0.30_{ 1.68}$,$ -4.49_{ 1.65}$ & 71.37 & 33.3 & 20.09 & 19.62 & 18.11 & & & & & & & & & $+10.56$ & 3.369 & \\
 4096107874989915648 & & $ 1.991_{ 0.367}$ & $ -1.90_{ 1.28}$,$ -2.40_{ 1.24}$ & 95.02 & 44.3 & & 19.58 & & & & & & & & & &  & & \\
\hline \noalign{\smallskip}
\textbf{\object{XX Sgr}} & 0.733 & $ 0.731_{ 0.059}$ & $ -0.05_{ 0.10}$,$ -0.48_{ 0.09}$ & & & 9.23 & 8.54 & 7.68 & 6.46 & 5.94 & 5.72 & 5.57 & 5.39 & 5.63 & 5.71 & 0.543 & $ -3.47$ & 3.770 & \\
 4096979650283681408 & & $ 0.697_{ 0.070}$ & $ +0.68_{ 0.50}$,$ -1.85_{ 0.35}$ & 7.87 & 10.7 & & 15.24 & & & & & & & & & &  & & \\
\hline \noalign{\smallskip}
\textbf{\object{AP Sgr}} & 1.287 & $ 1.148_{ 0.053}$ & $ +0.88_{ 0.16}$,$ -3.85_{ 0.13}$ & & & 7.46 & 6.90 & 6.24 & 5.27 & 4.98 & 4.78 & 4.77 & 4.71 & 4.86 & 4.84 & 0.192 & $ -3.27$ & 3.747 & \\
 4066429101224454144 & & $ 1.174_{ 0.187}$ & $ -1.86_{ 0.69}$,$ -3.42_{ 0.65}$ & 63.02 & 49.0 & 19.43 & 18.73 & 17.26 & & & & & & & & & $ +8.68$ & 3.141 & \\
 4066428998145128064 & & $ 1.249_{ 0.284}$ & $ -0.83_{ 0.82}$,$ -6.67_{ 0.76}$ & 36.28 & 28.2 & & 19.37 & & & & & & & & & &  & & \\
\hline \noalign{\smallskip}
\textbf{\object{V0950 Sco}} & 1.073 & $ 0.869_{ 0.052}$ & $ -0.48_{ 0.10}$,$ -1.66_{ 0.09}$ & & & 7.49 & 7.06 & 6.44 & 5.72 & 5.44 & 5.24 & 5.18 & 5.03 & 5.17 & 5.09 & 0.254 & $ -3.91$ & 3.784 & \\
 5960623340819585792 & & $ 1.149_{ 0.371}$ & $ +3.13_{ 1.00}$,$ -1.53_{ 0.94}$ & 16.93 & 15.8 & 17.93 & 17.79 & 16.73 & 12.81 & 13.35 & 13.18 & & & & & & $ +7.45$ & 3.764 & \\
 5960623340819009024 & & $ 1.148_{ 0.141}$ & $ -1.65_{ 0.38}$,$ -6.85_{ 0.32}$ & 29.33 & 27.3 & 18.83 & 18.40 & 17.24 & & & & & & & & & $ +8.11$ & 3.673 & \\
\hline \noalign{\smallskip}
\textbf{\object{Y Sct}} & 0.581 & $ 0.458_{ 0.067}$ & $ -0.68_{ 0.10}$,$ -3.08_{ 0.08}$ & & & 9.83 & 8.86 & 7.85 & 6.48 & 5.85 & 5.59 & 5.49 & 5.39 & 5.61 & 5.35 & 0.619 & $ -4.25$ & 3.702 & \\
 4156450099579515904 & & $ 0.663_{ 0.123}$ & $ -1.97_{ 0.29}$,$ -3.61_{ 0.26}$ & 28.38 & 48.8 & 18.40 & 17.23 & 16.08 & 14.49 & 14.06 & 13.67 & & & & & & $ +5.02$ & 3.530 & \\
\hline \noalign{\smallskip}
\textbf{\object{R TrA}} & 1.733 & $ 1.504_{ 0.037}$ & $ -5.23_{ 0.04}$,$ -8.31_{ 0.07}$ & & & 6.90 & 6.44 & 5.88 & 5.34 & 5.01 & 4.85 & 4.76 & 4.55 & 4.73 & 4.70 & 0.172 & $ -3.11$ & 3.772 & \\
 5824464631144871424 & & $ 1.567_{ 0.364}$ & $ -5.10_{ 0.52}$,$ -6.33_{ 0.77}$ & 56.57 & 32.6 & 19.82 & 19.31 & 18.45 & & & & & & & & & $ +9.87$ & 3.708 & \\
\hline \noalign{\smallskip}
\textbf{\object{LR TrA}} & 1.048 & $ 0.918_{ 0.032}$ & $ -4.86_{ 0.04}$,$ -7.87_{ 0.05}$ & & & 8.01 & 7.60 & 7.02 & 6.31 & 6.02 & 5.88 & 5.85 & 5.77 & 5.84 & 5.79 & 0.154 & $ -2.98$ & 3.772 & \\
 5824226655600814976 & & $ 1.005_{ 0.187}$ & $ -5.77_{ 0.24}$,$ -8.84_{ 0.39}$ & 37.56 & 35.8 & 19.94 & 19.00 & 17.96 & 16.64 & 15.43 & 15.01 & & & & & & $ +8.68$ & 3.303 & \\
   \hline
\end{tabular}
\end{sidewaystable*}



==> Tables/RRL-bound-table.tex <==
\begin{sidewaystable*}
\tiny
 \caption{Candidate gravitationally bound companions of RR Lyrae stars.
 The RR subtype is taken from the VSX database \citepads{2006SASS...25...47W}.
 The references for the photometry are given in the caption of Table~\ref{cepheids-bound-table1}.
 }
 \label{rrlyrae-bound-table}
 \centering
 \renewcommand{\arraystretch}{1}
\setlength\tabcolsep{4.5pt}
 \begin{tabular}{lrcrrrrrrrrrrrrrrcll}
 \hline
\hline \noalign{\smallskip}
RRL name / GDR2 & $\varpi_\mathrm{G2}$ & $\mu_{\alpha,\mathrm{G2}},\,\mu_{\delta,\mathrm{G2}}$ & Sep. & Sep. & $G_\mathrm{BP}$ & $G$ & $G_\mathrm{RP}$ & $J$ & $H$ & $K$ & $W1$ & $W2$ & $W3$ & $W4$ & $E(B-V)$ & $M_G$ & $\mathrm{Log}\,T$ & RR \\
 & (mas) & (mas\,a$^{-1}$) & ($\arcsec$) & (kau) & & & & & & & & & & & & & & type \\
\hline \noalign{\smallskip}
\textbf{\object{OV And}} & $ 0.938_{ 0.038}$ & $ -4.90_{ 0.06}$,$ -7.78_{ 0.03}$  &  &  & 11.93 & 11.34 & 10.64 &  9.68 &  9.15 &  9.00 &  8.91 &  8.99 &  8.91 &  8.53 & 0.053$^a$ & $ +1.08$ & 3.683 & RRab \\
 380489851377596928 &  $0.909_{ 0.039}$ & $ -4.43_{ 0.04}$,$ -7.71_{ 0.03}$ &   3.43 &   3.7 & 13.79 & 13.54 & 13.02 &  &  &  &  &  &  &  &  & $ +3.20$ & 3.781 & F4V \\
\hline \noalign{\smallskip}
\textbf{\object{CS Del}} & $0.635_{0.031}$ & $ -0.32_{ 0.05}$,$ +2.16_{ 0.06}$ & & & 13.05 & 12.85 & 12.50 & 12.02 & 11.88 & 11.83 & 11.74 & 11.79 & 11.78 & 9.07 & 0.095$^a$ & $+1.60$ & 3.830 & RRc \\
 1805526185917504512 & $0.644_{0.056}$ & $ -0.28_{ 0.10}$,$ +2.19_{ 0.10}$ & 3.17 & 5.0 & 16.32 & 16.14 & 15.42 & & & & & & & & & $+4.93$ & 3.774 & G7V \\
\hline \noalign{\smallskip}
\textbf{\object{V0893 Her}} & $2.679_{0.028}$ & $ -6.75_{ 0.05}$,$+11.54_{ 0.06}$ & & & 9.33 & 9.16 & 8.84 & 8.45 & 8.32 & 8.26 & 8.25 & 8.26 & 8.22 & 8.02 & 0.022$^a$ & $+1.24$ & 3.818 & RR: \\
 1385661079389302144 & $2.905_{0.443}$ & $ -9.68_{ 1.14}$,$+14.08_{ 1.20}$ & 5.16 & 1.9 & 16.19 & 16.65 & 15.09 & & & & & & & & & $+8.91$ & 3.725 & M1.5V \\
\hline \noalign{\smallskip}
\textbf{\object{RR Leo}} & $1.032_{0.088}$ & $-15.29_{ 0.10}$,$-10.16_{ 0.10}$ & & & 11.12 & 10.91 & 10.48 & 9.92 & 9.68 & 9.64 & 9.63 & 9.63 & 9.58 & 8.25 & 0.037$^b$ & $+0.87$ & 3.795 & RRab \\
 630421931138065280 & $1.062_{0.163}$ & $-16.30_{ 0.44}$,$-10.15_{ 0.32}$ & 9.64 & 9.3 & 18.74 & 18.05 & 17.16 & 15.97 & 15.31 & 15.11 & & & & & & $+8.10$ & 3.523 & M0V \\
\hline \noalign{\smallskip}
\textbf{\object{SS Oct}} & $0.862_{0.023}$ & $ -1.90_{ 0.05}$,$-32.70_{ 0.05}$ & & & 12.17 & 11.79 & 11.11 & 10.05 & 9.83 & 9.75 & 9.73 & 9.71 & 9.66 & 9.27 & 0.285$^b$ & $+0.73$ & 3.789 & RRab \\
 6345324695303800192 & $0.782_{0.114}$ & $ -2.22_{ 0.32}$,$-32.85_{ 0.24}$ & 2.67 & 3.1 & 16.80 & 17.18 & 15.80 & & & & & & & & & $+5.90$ & 3.797 & K2V \\
\hline \noalign{\smallskip}
\textbf{\object{EY Oph}} & $ 0.658_{ 0.032}$ & $ -2.64_{ 0.06}$,$ -1.75_{ 0.04}$  &  &  & 14.00 & 13.55 & 12.92 & 12.48 & 12.13 & 12.07 & 11.41 & 11.49 & 11.57 &  8.49 & 0.200$^a$ & $ +2.12$ & 3.769 & RR: \\
 6029835295648727168 &  $ 1.597_{ 0.341}$ & $ -4.52_{ 0.81}$,$ -4.26_{ 0.52}$ &  12.21 &   6.6 & 19.45 & 19.43 & 18.16 &  &  &  &  &  &  &  &  & $ +9.95$ & 3.738 & M3V (WD?)  \\
\hline \noalign{\smallskip}
\textbf{\object{V0487 Sco}} & $ 1.069_{ 0.075}$ & $ -9.83_{ 0.15}$,$-12.30_{ 0.12}$  &  &  & 11.54 & 11.22 & 10.67 &  9.90 &  9.65 &  9.60 &  8.14 &  8.20 &  8.30 &  8.67 & 0.252$^b$ & $+0.69$ & 3.811 & RRc \\
 4053551410541112192 &  $ 0.942_{ 0.060}$ & $-10.60_{ 0.12}$,$-12.61_{ 0.10}$ &  29.59 &  27.7 & 16.85 & 15.95 & 14.90 & 12.04 & 10.62 & 10.16 &  9.85 &  9.98 &  9.92 &  8.68 &  & $+5.26$ & 3.458 & dusty M giant ? \\
\hline
\end{tabular}
\tablebib{(a): 3D map \texttt{Bayestar17} by \citetads{2018MNRAS.478..651G}; (b): \citetads{2008MNRAS.386.2115F}. }
\end{sidewaystable*}



==> Tables/RRL-near-table.tex <==
\begin{sidewaystable*}
 \caption{Candidate \texttt{Near} companions of stars of RR Lyrae type in the GCVS \citepads{2009yCat....102025S}.
 EY Oph also has a candidate \texttt{Bound} companion listed in Table~\ref{rrlyrae-bound-table}.}
 \label{rrl-near-table1}
 \centering
\tiny
 \renewcommand{\arraystretch}{1}
\setlength\tabcolsep{4.5pt}
 \begin{tabular}{lrcrrrrrrrrrrrrrrcll}
 \hline
\hline \noalign{\smallskip}
RRL name / GDR2 & $\varpi_\mathrm{G2}$ & $\mu_{\alpha,\mathrm{G2}},\,\mu_{\delta,\mathrm{G2}}$ & Sep. & Sep. & $G_\mathrm{BP}$ & $G$ & $G_\mathrm{RP}$ & $J$ & $H$ & $K$ & $W1$ & $W2$ & $W3$ & $W4$ & $E(B-V)$ & $M_G$ & $\mathrm{Log}\,T$ & RR \\
 & (mas) & (mas\,a$^{-1}$) & ($\arcsec$) & (kau) & & & & & & & & & & & & & & type \\
\hline \noalign{\smallskip}
\textbf{\object{V0830 Cyg}} & $ 0.618_{ 0.019}$ & $ -1.59_{ 0.04}$,$ -1.98_{ 0.04}$ & & & 13.71 & 13.24 & 12.59 & 11.69 & 11.39 & 11.27 & 11.26 & 11.26 & 11.17 & 8.89 & 0.363 & $ +1.25$ & 3.796 & AB \\
 1873027163251912192 & $ 0.600_{ 0.124}$ & $ -3.35_{ 0.30}$,$ -4.12_{ 0.30}$ & 11.55 & 18.7 & 19.27 & 18.63 & 17.69 & 16.28 & 15.81 & 16.06 & & & & & & $ +6.65$ & 3.722 & \\
\hline \noalign{\smallskip}
\textbf{\object{CZ Lac}} & $ 0.852_{ 0.029}$ & $ -2.55_{ 0.06}$,$ -1.59_{ 0.05}$ & & & 11.95 & 11.69 & 11.18 & 10.82 & 10.60 & 10.53 & 10.28 & 10.27 & 10.20 & 8.98 & 0.065 & $ +1.17$ & 3.784 & AB \\
 2000976545410515584 & $ 0.773_{ 0.050}$ & $ -1.20_{ 0.09}$,$ -2.33_{ 0.08}$ & 21.05 & 24.7 & 16.94 & 16.42 & 15.78 & 15.05 & 14.56 & 14.49 & 14.22 & 14.33 & 12.72 & 9.24 & & $ +5.70$ & 3.722 & \\
\hline \noalign{\smallskip}
\textbf{\object{V0424 Lyr}} & $ 1.579_{ 0.187}$ & $ -0.41_{ 0.35}$,$ -4.72_{ 0.41}$ & & & 15.61 & 15.26 & 14.63 & 14.00 & 13.66 & 13.51 & 13.36 & 13.38 & 12.86 & 9.19 & 0.141 & $ +5.89$ & 3.771 & AB \\
 2036210631733553152 & $ 1.459_{ 0.209}$ & $ +1.37_{ 0.37}$,$ -4.99_{ 0.57}$ & 31.17 & 19.7 & 20.51 & 19.26 & 18.16 & 16.46 & 16.18 & 15.59 & 15.61 & 16.40 & 12.32 & 9.10 & & $ +9.80$ & 2.802 & \\
\hline \noalign{\smallskip}
\textbf{\object{AG Nor}} & $ 0.978_{ 0.093}$ & $ -4.49_{ 0.14}$,$ -5.71_{ 0.14}$ & & & 12.16 & 9.57 & 8.21 & 5.47 & 4.40 & 4.04 & 3.89 & 3.82 & 3.67 & 3.28 & & & & AB \\
 5835953600010583296 & $ 0.991_{ 0.198}$ & $ -4.59_{ 0.37}$,$ -4.83_{ 0.43}$ & 23.27 & 23.8 & 19.20 & 18.67 & 17.57 & & & & & & & & & & & \\
 5835953703089735552 & $ 1.100_{ 0.255}$ & $ -5.79_{ 0.47}$,$ -3.92_{ 0.55}$ & 12.59 & 12.9 & 19.45 & 18.67 & 16.83 & & & & & & & & & & & \\
 5835953668729965568 & $ 0.966_{ 0.154}$ & $ -2.96_{ 0.31}$,$ -4.91_{ 0.34}$ & 17.33 & 17.7 & 18.62 & 18.24 & 17.20 & 14.62 & 14.44 & 14.02 & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{KP Nor}} & $ 0.520_{ 0.054}$ & $ -1.76_{ 0.09}$,$ -3.92_{ 0.08}$ & & & 16.77 & 16.37 & 15.70 & 14.86 & 14.59 & 14.43 & 13.83 & 14.14 & 12.32 & 8.44 & & & & \\
 5831240057986282624 & $ 0.585_{ 0.124}$ & $ -1.03_{ 0.25}$,$ -2.53_{ 0.23}$ & 3.96 & 7.6 & 18.94 & 18.30 & 17.45 & 16.29 & 14.64 & 14.43 & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{EY Oph}} & $ 0.658_{ 0.032}$ & $ -2.64_{  0.06}$,$ -1.75_{  0.04}$  &  &  & 14.00 & 13.55 & 12.92 & 12.48 & 12.13 & 12.07 & 11.41 & 11.49 & 11.57 &  8.49 & 0.200 & $ +2.12$ & 3.769 & : \\
 6029835364429606784 &  $ 1.801_{ 0.419}$ & $ -7.11_{  0.81}$,$ -3.89_{  0.58}$ &  47.01 &  25.4 & 19.29 & 19.24 & 18.35 &    &    &    &    &    &    &    &  & $ +9.99$ & 3.787 &  \\
\hline \noalign{\smallskip}
\textbf{\object{IT Oph}} & $ 6.206_{ 0.045}$ & $ -0.92_{ 0.10}$,$-19.56_{ 0.06}$ & & & 13.58 & 12.75 & 11.81 & 10.27 & 9.30 & 8.59 & 7.85 & 7.28 & 5.61 & 3.64 & 0.032 & $ +6.64$ & 3.349 & \\
 4108442162053920640 & $ 5.602_{ 0.813}$ & $ -0.73_{ 2.87}$,$ -5.72_{ 1.93}$ & 150.54 & 24.3 & & 20.06 & & & & & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{MS Oph}} & $ 0.658_{ 0.146}$ & $ +3.36_{ 0.24}$,$ -0.60_{ 0.16}$ & & & 14.33 & 11.33 & 9.86 & 7.01 & 6.02 & 5.59 & 5.48 & 5.35 & 0.00 & 3.72 & 0.148 & $ +0.19$ & -1.535 & : \\
 6029618245128099200 & $ 0.604_{ 0.070}$ & $ +4.91_{ 0.13}$,$ -0.20_{ 0.08}$ & 8.16 & 12.4 & 17.04 & 16.56 & 15.84 & & & & & & & & & $ +5.09$ & 3.739 & \\
\hline \noalign{\smallskip}
\textbf{\object{V1693 Oph}} & $ 0.677_{ 0.340}$ & $ +0.26_{ 1.30}$,$ -7.16_{ 0.99}$ & & & & 19.61 & & 15.75 & 15.19 & 14.98 & & & & & 0.219 & & & AB \\
 4134311639114110464 & $ 0.592_{ 0.071}$ & $ +0.59_{ 0.19}$,$ -2.04_{ 0.12}$ & 19.58 & 28.9 & 17.37 & 16.82 & 16.10 & 15.17 & 14.67 & 14.54 & 14.18 & 14.16 & 11.96 & 8.81 & & $ +5.14$ & 3.744 & \\
\hline \noalign{\smallskip}
\textbf{\object{UY Ori}} & $ 2.840_{ 0.082}$ & $ +1.78_{ 0.18}$,$ +0.96_{ 0.12}$ & & & 12.49 & 12.40 & 12.13 & 11.48 & 10.51 & 9.33 & 7.86 & 6.94 & 3.11 & 1.24 & 0.164 & $ +4.19$ & 3.945 & : \\
 3209513031759316736 & $ 2.593_{ 0.449}$ & $ +5.73_{ 1.38}$,$ -2.05_{ 1.22}$ & 24.77 & 8.7 & 20.93 & 19.97 & 18.58 & 16.92 & 15.81 & 15.15 & & & & & & $+11.71$ & 2.855 & \\
\hline \noalign{\smallskip}
\textbf{\object{V1154 Ori}} & $ 1.087_{ 0.054}$ & $ -1.47_{ 0.10}$,$ -2.21_{ 0.09}$ & & & 10.94 & 10.87 & 10.71 & 10.48 & 10.44 & 10.37 & 10.31 & 10.34 & 10.08 & 5.70 & 0.267 & $ +0.25$ & 4.181 & C \\
 3345190391512281600 & $ 0.993_{ 0.045}$ & $ -0.81_{ 0.08}$,$ -1.53_{ 0.08}$ & 28.28 & 26.0 & 11.82 & 11.77 & 11.60 & 11.39 & 11.39 & 11.33 & 11.25 & 11.30 & 10.62 & 5.40 & & $ +0.94$ & 4.186 & \\
\hline \noalign{\smallskip}
\textbf{\object{V0701 Sgr}} & $ 2.000_{ 0.302}$ & $ +2.84_{ 0.69}$,$ +0.43_{ 0.63}$ & & & 13.94 & 13.65 & 13.08 & 12.25 & 11.99 & 11.90 & 11.88 & 11.94 & 11.38 & 8.04 & & & & AB \\
 4038120868676971008 & $ 2.117_{ 0.349}$ & $ +1.59_{ 0.85}$,$ -3.41_{ 0.78}$ & 54.71 & 27.4 & 19.54 & 19.35 & 17.91 & 16.02 & 15.58 & 15.39 & 15.05 & 16.84 & 11.85 & 8.91 & & & & \\
 4038120971756176128 & $ 2.036_{ 0.224}$ & $ +1.15_{ 0.54}$,$ -0.98_{ 0.49}$ & 43.74 & 21.9 & 19.07 & 18.94 & 17.91 & & & & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{V2481 Sgr}} & $ 0.910_{ 0.197}$ & $ +3.27_{ 0.65}$,$ -1.10_{ 0.54}$ & & & 15.60 & 14.72 & 13.56 & 12.15 & 11.14 & 11.02 & & & & & 0.107 & $ +4.29$ & 3.161 & C: \\
 4062366092483595776 & $ 0.974_{ 0.150}$ & $ -0.05_{ 0.49}$,$ -0.70_{ 0.41}$ & 25.76 & 28.3 & 16.89 & 16.68 & 15.64 & & & & & & & & & $ +6.36$ & 3.717 & \\
\hline \noalign{\smallskip}
\textbf{\object{V2626 Sgr}} & $ 1.363_{ 0.047}$ & $ +4.15_{ 0.08}$,$ -1.40_{ 0.07}$ & & & 15.39 & 14.94 & 14.31 & 13.57 & 13.18 & 13.12 & 12.86 & 13.04 & 11.78 & 8.25 & & & & AB \\
 4039178186528038400 & $ 1.203_{ 0.245}$ & $ +3.46_{ 0.50}$,$ -0.66_{ 0.45}$ & 22.13 & 16.2 & & 18.90 & & 15.95 & 15.10 & 15.08 & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{V3531 Sgr}} & $ 0.766_{ 0.462}$ & $ -1.14_{ 0.96}$,$ -3.00_{ 0.81}$ & & & 17.19 & 17.01 & 16.26 & 15.43 & 15.03 & 15.04 & & & & & & & & AB \\
 4046831577743784192 & $ 0.748_{ 0.150}$ & $ +2.36_{ 0.31}$,$ -2.71_{ 0.26}$ & 10.82 & 14.1 & 17.91 & 17.63 & 16.87 & 16.17 & 15.80 & 15.07 & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{V4107 Sgr}} & $ 1.265_{ 0.142}$ & $ -3.28_{ 0.40}$,$ -1.74_{ 0.34}$ & & & 16.81 & 16.61 & 15.55 & & & & & & & & 0.113 & $ +6.84$ & 3.715 & AB \\
 4050225564037689472 & $ 1.404_{ 0.254}$ & $ -4.61_{ 0.53}$,$ -4.06_{ 0.49}$ & 36.78 & 29.1 & 18.08 & 18.12 & 16.57 & & & & & & & & & $ +8.59$ & 3.630 & \\
\hline \noalign{\smallskip}
\textbf{\object{V4313 Sgr}} & $ 1.700_{ 0.282}$ & $ -3.98_{ 0.68}$,$ -1.83_{ 0.57}$ & & & 16.20 & 16.22 & 15.31 & 14.32 & 14.04 & 14.00 & & & & & 0.087 & $ +7.14$ & 3.772 & AB \\
 4049184322231156736 & $ 1.702_{ 0.230}$ & $ -3.80_{ 0.58}$,$ +0.79_{ 0.48}$ & 47.85 & 28.2 & 17.90 & 17.48 & 16.43 & & & & & & & & & $ +8.43$ & 3.629 & \\
 4049184425310375808 & $ 1.869_{ 0.326}$ & $ -1.86_{ 0.72}$,$ -3.94_{ 0.72}$ & 28.12 & 16.5 & & 18.91 & & 13.15 & 12.53 & 12.34 & 10.90 & 11.17 & 10.93 & 8.06 & & & & \\
\hline
\end{tabular}
\end{sidewaystable*}




\begin{sidewaystable*}
 \caption{Continued from Table~\ref{rrl-near-table1}.}
 \label{rrl-near-table2}
  \centering
\tiny
 \renewcommand{\arraystretch}{1}
 \setlength\tabcolsep{4.5pt}
\begin{tabular}{lrcrrrrrrrrrrrrrrcll}
 \hline
\hline \noalign{\smallskip}
RRL name / GDR2 & $\varpi_\mathrm{G2}$ & $\mu_{\alpha,\mathrm{G2}},\,\mu_{\delta,\mathrm{G2}}$ & Sep. & Sep. & $G_\mathrm{BP}$ & $G$ & $G_\mathrm{RP}$ & $J$ & $H$ & $K$ & $W1$ & $W2$ & $W3$ & $W4$ & $E(B-V)$ & $M_G$ & $\mathrm{Log}\,T$ & RR \\
 & (mas) & (mas\,a$^{-1}$) & ($\arcsec$) & (kau) & & & & & & & & & & & & & & type \\
\hline \noalign{\smallskip}
\textbf{\object{V4355 Sgr}} & $ 2.433_{ 0.313}$ & $ +0.13_{ 0.69}$,$ -3.87_{ 0.61}$ & & & 16.48 & 16.20 & 15.42 & 14.60 & 14.27 & 14.05 & & & & & & & & AB \\
 4048847360538237696 & $ 2.357_{ 0.538}$ & $ -3.29_{ 1.41}$,$ -3.73_{ 1.27}$ & 69.70 & 28.6 & & 19.60 & & 15.19 & 14.69 & 14.42 & & & & & & & & \\
 4048847704135531136 & $ 2.484_{ 0.404}$ & $ -1.82_{ 1.17}$,$ -6.79_{ 1.03}$ & 34.25 & 14.1 & 19.43 & 19.31 & 18.15 & & & & & & & & & & & \\
 4048847772895728000 & $ 2.131_{ 0.415}$ & $ -3.41_{ 0.89}$,$ -3.50_{ 1.00}$ & 47.67 & 19.6 & 19.07 & 19.19 & 17.66 & & & & & & & & & & & \\
 4048847734320589312 & $ 2.100_{ 0.359}$ & $ -2.61_{ 0.99}$,$ -4.08_{ 0.97}$ & 40.85 & 16.8 & & 19.14 & & & & & & & & & & & & \\
 4048847803040124416 & $ 2.691_{ 0.434}$ & $ -3.75_{ 1.11}$,$ -3.50_{ 1.04}$ & 64.61 & 26.6 & 18.62 & 19.25 & 17.45 & & & & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{V4591 Sgr}} & $ 1.837_{ 0.179}$ & $ -0.34_{ 0.46}$,$ -2.21_{ 0.38}$ & & & 17.67 & 17.29 & 16.34 & 15.51 & 14.80 & 14.62 & & & & & & & & AB \\
 4048827462005964416 & $ 1.821_{ 0.303}$ & $ -1.50_{ 0.67}$,$ -6.42_{ 0.60}$ & 26.75 & 14.6 & 19.23 & 18.93 & 17.68 & & & & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{IY Sco}} & $ 2.530_{ 0.042}$ & $ -8.94_{ 0.06}$,$ -4.25_{ 0.05}$ & & & 14.07 & 13.59 & 12.95 & 12.17 & 11.78 & 11.66 & 11.58 & 11.67 & 11.51 & 8.82 & & & & \\
 6028393767161904000 & $ 2.276_{ 0.516}$ & $ -8.19_{ 1.38}$,$ -1.00_{ 0.88}$ & 67.23 & 26.6 & 19.93 & 19.81 & 18.72 & & & & & & & & & & & \\
 6028394007680341248 & $ 2.641_{ 0.513}$ & $ -3.55_{ 1.70}$,$ -0.40_{ 1.15}$ & 30.23 & 11.9 & 19.05 & 19.87 & 18.58 & & & & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{KN Sco}} & $ 0.959_{ 0.043}$ & $ -0.60_{ 0.07}$,$ -2.42_{ 0.05}$ & & & 14.22 & 13.79 & 13.21 & 12.34 & 12.09 & 11.98 & 11.74 & 11.77 & 12.05 & 8.47 & 0.423 & $ +2.56$ & 3.841 & \\
 6028937883678549888 & $ 1.077_{ 0.199}$ & $ +0.02_{ 0.48}$,$ -4.26_{ 0.32}$ & 27.43 & 28.6 & 19.34 & 18.66 & 17.71 & & & & & & & & & $ +7.82$ & 3.728 & \\
\hline \noalign{\smallskip}
\textbf{\object{V0828 Sco}} & $ 0.877_{ 0.435}$ & $ -6.58_{ 1.89}$,$ -8.06_{ 1.77}$ & & & & 19.07 & & 14.62 & 14.28 & 14.42 & & & & & & & & \\
 5954643058331900160 & $ 0.871_{ 0.124}$ & $ -8.88_{ 0.33}$,$ -5.36_{ 0.30}$ & 22.86 & 26.1 & 18.70 & 18.06 & 17.34 & 16.41 & 15.51 & 15.56 & & & & & & & & \\
\hline \noalign{\smallskip}
\textbf{\object{V0348 Sct}} & $ 1.249_{ 0.042}$ & $ -1.36_{ 0.06}$,$ +0.51_{ 0.05}$ & & & 13.56 & 13.17 & 12.61 & 11.94 & 11.66 & 11.57 & 11.51 & 11.51 & 11.97 & 8.74 & 0.109 & $ +3.37$ & 3.768 & \\
 4203792424572067968 & $ 1.096_{ 0.161}$ & $ -3.73_{ 0.52}$,$ +1.42_{ 0.43}$ & 26.44 & 21.2 & 18.94 & 18.16 & 17.24 & 15.91 & 15.36 & 15.03 & & & & & & $ +8.11$ & 3.507 & \\
\hline
\end{tabular}
%\tablebib{(a): 3D map \texttt{Bayestar17} by \citetads{2018MNRAS.478..651G}; (b): \citetads{2008MNRAS.386.2115F}. }
\end{sidewaystable*}


==> Tables/VAR-bound-table.tex <==
\begin{sidewaystable*}
\caption{Candidate gravitationally bound companions of various variable stars. The references for the photometry are given in the caption of Table~\ref{cepheids-bound-table1}.}
\label{various-bound-table}
\centering
\tiny
\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{4.5pt}
\begin{tabular}{lrcrrrrrrrrrrrrrrcll}
\hline
\hline \noalign{\smallskip}
Star name / GDR2 & $\varpi_\mathrm{G2}$ & $\mu_{\alpha,\mathrm{G2}},\,\mu_{\delta,\mathrm{G2}}$ & Sep. & Sep. & $G_\mathrm{BP}$ & $G$ & $G_\mathrm{RP}$ & $J$ & $H$ & $K$ & $W1$ & $W2$ & $W3$ & $W4$ & $E(B-V)$ & $M_G$ & $\mathrm{Log}\,T$ & Type \\
 & (mas) & (mas\,a$^{-1}$) & ($\arcsec$) & (kau) & & & & & & & & & & & & &  \\
\hline \noalign{\smallskip}
\textbf{\object{HM Aql}} & $1.829_{0.037}$ & $ +0.65_{ 0.07}$,$ -5.85_{ 0.06}$ & & & 13.54 & 12.85 & 12.02 & 10.85 & 10.49 & 10.34 & & & & & 0.616$^a$ & $+2.62$ & 3.789 & F1V, ? \\
 4259109541759198848 & $1.709_{0.105}$  & $ +0.42_{ 0.23}$,$ -6.37_{ 0.21}$& 26.84 & 14.7 & 19.09 & 17.49 & 16.24 & 14.06 & 13.12 & 12.81 & & & & & & $+7.44$ & (2.971) & K7V \\
\hline \noalign{\smallskip}
\textbf{\object{EN CMi}} & $ 0.569_{0.066}$ & $ -3.70_{ 0.13}$,$ +2.24_{ 0.08}$ & & & 17.10 & 16.66 & 16.06 & 15.39 & 15.08 & 14.86 & 14.68 & 14.78 & 12.38 & 8.22 & 0.037$^a$ & $ +5.34$ & 3.741 & G9V, ? \\
 3083253225327313024 & $ 0.519_{0.091}$ & $ -4.30_{ 0.20}$,$ +2.72_{ 0.11}$ & 13.84 & 24.3 & 17.57 & 17.16 & 16.62 & 16.10 & 15.58 & 15.22 & 15.58 & 15.76 & 12.51 & 8.71 & & $ +5.64$ & 3.755 & K1.5V \\
\hline \noalign{\smallskip}
\textbf{\object{NQ Cyg}} & $ 0.938_{0.093}$ & $ -5.86_{ 0.21}$,$-11.20_{ 0.20}$ & & & 16.33 & 16.37 & 16.05 & 15.14 & 14.92 & 14.78 & & & & & 0.082$^a$ & $ +5.99$ & 3.916 & K2.5V, Ecl. binary$^c$ \\
 2072926589158425856 & $ 0.932_{0.106}$ & $ -5.25_{ 0.25}$,$ -9.94_{ 0.25}$ & 18.20 & 19.4 & 18.93 & 18.17 & 17.34 & 16.35 & 15.69 & 15.41 & & & & & & $ +7.83$ & 3.556 & K9V \\
\hline \noalign{\smallskip}
\textbf{\object{V1391 Cyg}} & $1.232_{0.056}$ & $ -1.17_{ 0.11}$,$ -3.76_{ 0.12}$ & & & 16.47 & 15.42 & 14.38 & 12.68 & 11.86 & 11.56 & 11.21 & 10.91 & 8.16 & 5.84 & 0.216$^a$ & $+5.42$ & 3.268 & K0V, Ecl. binary$^d$ \\
 2067355638620630912 & $1.057_{0.183}$ & $ -1.32_{ 0.42}$,$ -3.90_{ 0.56}$ & 3.57 & 2.9 & 20.50 & 19.22 & 17.63 & & & & & & & & & $+8.94$ & (2.077) & M1.5V \\
\hline \noalign{\smallskip}
\textbf{\object{V2121 Cyg}} & $25.597_{0.064}$ & $+68.69_{ 0.11}$,$+57.11_{ 0.13}$ & & & 5.82 & 5.66 & 5.37 & 5.35 & 5.01 & 4.91 & 4.91 & 4.73 & 4.96 & 4.91 & 0.004$^a$ & $+2.69$ & 3.822 & F1V, $\gamma$\,Dor$^e$ \\
 2084032103278208640 & $25.652_{0.029}$ & $+72.29_{ 0.06}$,$+53.72_{ 0.05}$ & 55.64 & 2.2 & 13.59 & 12.27 & 11.13 & 9.58 & 8.90 & 8.70 & 8.57 & 8.48 & 8.44 & 9.09 & & $+9.31$ & 2.279 & M2V \\
\hline \noalign{\smallskip}
\textbf{\object{UU Dor}} & $0.856_{0.060}$ & $ -2.26_{ 0.12}$,$ -0.75_{ 0.19}$ & & & 14.61 & 14.39 & 13.84 & 13.41 & 13.11 & 13.03 & 12.73 & 12.75 & 11.67 & 9.58 & 0.159$^c$ & $+3.62$ & 3.805 & F6V, Ecl. binary$^f$ \\
 4657579638104003968 & $0.857_{0.098}$ & $ -1.55_{ 0.48}$,$ -0.87_{ 0.32}$ & 0.92 & 1.1 & & 16.90 & &  &  &  &  &  &  &  & & $+6.13$ & & K3V \\
\hline \noalign{\smallskip}
\textbf{\object{IW Lib}} & $3.571_{0.112}$ & $+10.95_{ 0.11}$,$ -5.18_{ 0.08}$ & & & 9.59 & 9.22 & 8.66 & 8.01 & 7.70 & 7.63 & 7.57 & 7.55 & 7.58 & 7.43 & 0.231$^a$ & $+1.37$ & 3.753 & A1V, W\,UMa ecl.$^g$ \\
 6234240520157591424 & $3.417_{0.063}$ & $+11.69_{ 0.08}$,$ -5.23_{ 0.06}$ & 17.27 & 4.8 & 15.26 & 14.48 & 13.62 & 12.43 & 11.77 & 11.69 & 11.33 & 11.32 & 11.29 & 8.92 & & $+6.62$ & 3.639 & K3V \\
\hline \noalign{\smallskip}
\textbf{\object{AZ Men}} & $1.088_{0.037}$ & $ -1.56_{ 0.04}$,$ -5.57_{ 0.04}$ & & & 14.15 & 13.81 & 13.30 & 12.61 & 12.33 & 12.22 & 12.29 & 12.30 & 12.10 & 9.28 & 0.114$^c$ & $+3.69$ & 3.782 & ?F7V,  \\
 4628608777985655296 & $1.159_{0.053}$ & $ -1.60_{ 0.10}$,$ -5.50_{ 0.11}$ & 16.71 & 15.4 & 17.46 & 16.77 & 15.98 & 14.97 & 14.39 & 14.29 & 14.17 & 14.22 & 13.19 & 9.63 & & $+6.82$ & 3.638 & K5V \\
\hline \noalign{\smallskip}
\textbf{\object{V1171 Oph}} & $1.098_{0.048}$ & $ -1.97_{ 0.07}$,$ -0.78_{ 0.05}$ & & & 14.09 & 13.70 & 13.13 & 12.40 & 12.08 & 11.96 & 11.81 & 11.84 & 11.46 & 8.86 & 0.237$^a$ & $+3.28$ & 3.792 & F8V, ? \\
 4129610367918498432 & $0.985_{0.071}$ & $ -2.17_{ 0.14}$,$ -1.10_{ 0.09}$ & 3.94 & 3.6 & 16.82 & 16.27 & 15.50 & 14.46 & 14.07 & 13.81 & & & & & & $+5.65$ & 3.740 & K1V \\
\hline \noalign{\smallskip}
\textbf{\object{V1330 Sgr}} & $ 1.229_{0.224}$ & $ -5.80_{ 0.45}$,$ -2.23_{ 0.37}$ & & & 17.32 & 16.92 & 15.70 & 14.12 & 13.27 & 13.00 & & & & & 0.191$^a$ & $ +6.93$ & 3.624 & K5V, ? \\
 4050169523277366656 & $ 1.398_{0.320}$ & $ -3.57_{ 0.61}$,$ -1.36_{ 0.51}$ & 30.35 & 24.7 & 18.33 & 17.86 & 16.42 & & & & & & & & & $ +8.17$ & 3.413 & M0V \\
\hline \noalign{\smallskip}
\textbf{\object{V1382 Sgr}} & $1.611_{0.280}$ & $ -3.95_{ 0.40}$,$ -5.42_{ 0.33}$ & & & 16.86 & 16.51 & 15.08 & 13.71 & 13.02 & 12.79 & & & & & 0.119$^a$ & $+7.28$ & 3.450 & K6V, ? \\
 4050171683873801216 & $1.719_{0.287}$ & $ -2.96_{ 0.54}$,$ -5.13_{ 0.46}$ & 18.71 & 11.6 & 18.49 & 18.33 & 16.77 & & & & & & & & & $+9.24$ & 3.500 & M2V \\
\hline \noalign{\smallskip}
\textbf{\object{V2248 Sgr}} & $1.948_{0.040}$ & $ +5.50_{ 0.05}$,$-11.43_{ 0.04}$ & & & 14.06 & 13.57 & 12.95 & 12.18 & 11.77 & 11.70 & 11.56 & 11.60 & 11.15 & 8.80 & 0.043$^b$ & $+4.92$ & 3.729 & G7V, W\,UMa ecl.$^h$ \\
 6694128163462947200 & $1.923_{0.048}$ & $ +5.39_{ 0.07}$,$-11.52_{ 0.06}$ & 53.54 & 27.5 & 16.01 & 15.35 & 14.59 & 13.66 & 13.05 & 12.89 & 12.87 & 12.89 & 12.39 & 8.85 & & $+6.67$ & 3.622 & K3.5V \\
\hline \noalign{\smallskip}
\textbf{\object{V3166 Sgr}} & $6.646_{0.070}$ & $ -0.97_{ 0.15}$,$-26.78_{ 0.12}$ & & & & 14.34 & & 10.60 & 9.78 & 9.37 & 8.67 & 8.20 & 6.61 & 4.50 & 0.030$^b$ & $+8.48$ & 3.488 & M0.5V, ? \\
 4044760647636888576 & $6.705_{0.053}$ & $ -3.27_{ 0.11}$,$-26.91_{ 0.09}$ & 1.64 & 0.2 & 14.86 & 13.73 & 12.43 &  &  &  &  &  &  &  & & $+7.81$ & (2.387) & K8V \\
 4044760643280597504 & $6.883_{0.098}$ & $ -2.31_{ 0.17}$,$-25.97_{ 0.14}$ & 9.00 & 1.4 & 16.57 & 14.73 & 13.42 & 11.46 & 10.82 & 10.60 & 10.37 & 10.15 & 10.20 & 8.11 & & $+8.87$ & 3.547 & M1V \\
\hline \noalign{\smallskip}
\textbf{\object{HR Sco}} & $7.370_{0.576}$ & $ -1.32_{ 1.20}$,$ +7.59_{ 0.70}$ & & & 16.13 & 15.89 & 14.94 & 13.91 & 13.50 & 13.57 & & & & & 0.010$^a$ & $+10.20$ & 3.683 & M3V, ? \\
 6029291827664185600 & $7.052_{1.490}$ & $ -2.30_{ 2.07}$,$ +5.53_{ 1.20}$ & 155.4 & 21.1 & 19.66 & 20.38 & 18.59 & & & & & & & & & $+14.60$ & 3.728 & M5V \\
\hline
\end{tabular}
\tablebib{(a): \citetads{2018MNRAS.478..651G};
(b): \citetads{2018A&A...616A.132L};
(c): \citetads{2017AstL...43..472G}, converted using $E(B-V)=1.655 \, E(J-K_S)$.
(d) \citetads{2014AJ....147..119C};
(e) \citetads{2005AJ....129.2815H};
(f) \citetads{2011AcA....61..103G};
(g) \citetads{2012ApJS..203...32R};
(h) \citetads{2005IBVS.5613....1A}.}
\end{sidewaystable*}
